PRISM: Progressive Restoration for Scene Graph-based Image Manipulation

Scene graphs have emerged as accurate descriptive priors for image generation and manipulation tasks, however, their complexity and diversity of the shapes and relations of objects in data make it challenging to incorporate them into the models and generate high-quality results. To address these challenges, we propose PRISM, a novel progressive multi-head image manipulation approach to improve the accuracy and quality of the manipulated regions in the scene. Our image manipulation framework is trained using an end-to-end denoising masked reconstruction proxy task, where the masked regions are progressively unmasked from the outer regions to the inner part. We take advantage of the outer part of the masked area as they have a direct correlation with the context of the scene. Moreover, our multi-head architecture simultaneously generates detailed object-specific regions in addition to the entire image to produce higher-quality images. Our model outperforms the state-of-the-art methods in the semantic image manipulation task on the CLEVR and Visual Genome datasets. Our results demonstrate the potential of our approach for enhancing the quality and precision of scene graph-based image manipulation.

==> chapters/temp.tex <==
Intro
 \iffalse (Many might not agree to the high-quality part, but maybe faster convergence? Maybe the firt part, talk about the architectures, and what kind of prior do they need to generate the images since the paper is also about multiple conditionings) \fi

\iffalse
The field of image generation and manipulation has seen significant advancements in recent years, with autoencoders \cite{VAE} and GANs \cite{GAN} being the primary approaches in the early years. Generator architectures have progressed substantially in complexity, with the development of architectures such as SPADE \cite{SPADE_2019} and Pix2Pix \cite{pix2pixHD_2018}. While recent research on diffusion models \cite{diffusion_original} has gained interest, GANs remain a popular choice due to their ability to achieve great performance in generating high-quality images. %\iffalse (Many might not agree to the high-quality part, but maybe faster convergence? Maybe the firt part, talk about the architectures, and what kind of prior do they need to generate the images since the paper is also about multiple conditionings)
%\fi


(first: image generation conditioned on the scene graphs, and then editing by text, scene graphs, etc. Why not having the input for both generation and editing.)\fi


\iffalse
%Despite the strenths of such methods, they face several challenges that limit their effectiveness. 
However, these methods tend to face several challenges that limit their effectiveness.
%due to the complexity and high diversity of the datasets such as visual genome, which can lead to poor quality results.
These challenges include insufficient context information during the training, the inherent complexity and diversity of the scenes in datasets such visual genome and the ambiguity of some relationships such as \textit{near} or \textit{by}. 
These limitations result in suboptimal image quality, making it challenging to use scene graph-based image generation and manipulation techniques for practical applications.
\fi


%Our approach builds on previous work in image manipulation and scene graph-based image generation. In particular, recent work has shown the potential of generative adversarial networks (GANs) for generating images from scene graphs. 
%However, these methods tend to suffer from limitations due to the complexity and high diversity of the datasets such as visual genome, which can lead to poor quality results. Other methods have explored the use of progressive image generation, which gradually adds details to the image during the generation process. However, these methods require direct supervision, making them less flexible and limiting their applicability to practical use cases.


% history
%As early as the 1960s, computer vision researchers experimented with the first methods for image manipulation tasks such as image restoration and image enhacement~\cite{CV_history}. Since then, there has been rapid progress due to deep learning methods which have transformed the computer vision research landscape~\cite{DeepLearning_LeCun2015,deep_learning_bengio}. The progress of deep learning methods has led us to generative models~\cite{Normalizing_flows_orig, VAE, GAN,diffusion_original} capable of manipulating and generating first semi-realistic images. Generative Adversarial Networks~\cite{GAN} or GANs for short in particular have transformed the computer vision research landscape through their potential to generate natural-looking images. With the GAN improvements in terms of training stability~\cite{DCGAN,improved_GANS_2016}, aided by newly introduced losses that focus on high-level differences between images~\cite{improved_GANS_2016,perceptual_johnson2016}, GANs have become models of choice for image generation and image manipulation tasks.\\


%GANs have been used in a number of image alteration tasks such as semantic image manipulation~\cite{sem_img_manipulation,simsg}, image inpainting~\cite{inpainting_pathak2016context,inpainting_dhamo_2019}, or image outpainting~\cite{scene_graph_outpainting}. There are two prevalent approaches to image manipulation tasks. First, an approach that generates images according to user modification specification done directly on the image~\cite{style_structure_wang_2016, SESAME,dalle2_ramesh2022}. Second, an approach that first generates an intermediate feature representation of an image, and then generates an image based on the user's intermediate representation modification of an image~\cite{simsg,scene_graph_outpainting,scene_graph_disentangled_azade2022}. 

% The most prominent feature representation is called a scene graph~\cite{scene_graphs_johnson2015}. Scene graphs are a structural representation of a scene typically in an image via graphs where a node in the graph usually represents an object. These nodes along with their corresponding attributes are encoded using a feature vector encoding and are connected via edges which signify a relationship or connection between the node objects. They encode spatial relationship information between objects and provide attribute binding for objects~\cite{scene_graphs_survey}. Having such a powerful representation allows the user to achieve a number of abstract modifications while simultaneously having a level of control unachievable by other approaches.\\


%In this work, we address the problem of image manipulation from scene graphs, in which a user can modify images by applying changes in the nodes or edges of the semantic graph representation of the image. This work builds upon the work of Dhamo et al. called Semantic Image Manipulation Using Scene Graphs~\cite{simsg}, or SIMSG for short. SIMSG offers a complete solution for image manipulation in low resolution. 
%To summarize our contribution:  First, we present a novel multi-task approach for image manipulation. The multi-task approach is realized through a Generative Adversarial Network (GAN) featuring a decoder comprised of two heads. One head focuses on generating detailed reconstruction of manipulated image parts while the other focuses on holistic image reconstruction. Second, we utilize a progressive restoration process for image reconstruction, which provides additional context information that enables more precise image manipulation. We analyze these techniques quantitatively in an image restoration task and qualitatively through performing image manipulation. Finally, we combine these techniques into a novel progressive multi-task image manipulation approach that significantly outperforms the state-of-the-art methods.



% The semantic generator produces a semantic map guided by a foreground object binary mask obtained from a two-headed network depicted in Fig.~\ref{fig:hierarch_mask_two_stream}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/semantic_image_manipulation_generator.pdf}
%     \caption[Architecture of structure generator by Hong et al.\ ]{The Structure generator architecture proposed by Hong et al.~\protect\cite{sem_img_manipulation}}\label{fig:hierarch_mask_two_stream}
% \end{figure}

% Images generated using DALLE-2 showcasing these limitations can be seen in Fig.~\ref{fig:dalle2_issues}. Both of these issues are not present when using a scene graph representation of an image.

% \begin{figure}[ht]
%     \centering
%     \subfloat[]{{\includegraphics[width=0.2\textwidth]{figures/dalle2_attribute.png}}}%
%     \quad
%     \subfloat[]{{\includegraphics[width=0.2\textwidth]{figures/dalle2_position.png}}}%
%     \caption[Images generated by DALLE-2 showcasing its limitations]{Result of DALLE-2 image generation given a query ``a white cube on top of a blue cube''. Showcasing object attribute-binding issues \textbf{(a)} and inability to reason about position \textbf{(b)}}%
%     \label{fig:dalle2_issues}%
% \end{figure}

% \begin{table}[ht]
% \centering
% \begin{tabular}{l|llll}
% \hline
%                       & MAE $\downarrow$      & SSIM $\uparrow$ & LPIPS $\downarrow$ & FID $\downarrow$ \\ \hline
% W/o Connection            & 4.888 &   0.985    &  0.011  &  2.702  \\
% With Connection            & \textbf{4.273}     & 0.985 & 0.011  &  \textbf{2.629}  \\ \hline
% \end{tabular}
% \caption[Ablation study between two-headed approach with and without connection on the CLEVR dataset]{Ablation study between two-headed approach with and without connection between the heads on the CLEVR dataset performed through image reconstruction}\label{tab:two_head_connection}
% \end{table}


 %We normalize each image per channel with the per-channel mean and variance of all the images in the ImageNet dataset~\cite{imagenet_2009}. Specifically, the output image is defined in \autoref{eq:norm_image}

%\begin{equation}\label{eq:norm_image}
%{Norm\_image}_{ch} = \dfrac{{Input\_img}_{ch} - {ImageNet\_mean}_{ch}}{{ImageNet\_std}_{ch}}
%\end{equation}

%, where $ch$ indicates per channel computation. Afterward, we resize the images into a $64\times 64$ dimension. Subsequently, the processed images are fed into a state-of-the-art scene graph prediction network called Factorizable Net~\cite{factorizable_net_2018}. 


%\footnotetext[3]{Profile available at \href{https://www.pexels.com/@drone-trotter-2765040/}{https://www.pexels.com/@drone-trotter-2765040/}}
%\footnotetext[4]{Image available at \href{https://www.pexels.com/photo/white-yacht-in-azure-sea-5640310/}{https://www.pexels.com/photo/white-yacht-in-azure-sea-5640310/}}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/progressive_baseline.pdf}
%     \caption[Architecture of the handcrafted progressive generation]{Architecture of the handcrafted progressive generation approach. The model progressively fills in the border regions of masked input by replacing the mask with generated image pixels.} 
%     %The RGB image was taken by Drone Trotter\protect\footnotemark on Pexels\protect\footnotemark}\label{fig:progressive_baseline}
%     \label{fig:prog}
% \end{figure}



\iffalse
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/two_heads_connection.pdf}
    \caption[Architecture of the multi-task two-headed approach]{Architecture of the multi-task two-headed approach. During training, the system takes masked input (on the left), uses a multi-step decoder to create a layout representation, and then through a series of SPADE~\cite{SPADE_2019} ResNet blocks reconstructs the entire original image (top-right) and detailed reconstruction of the masked object (bottom-right).} %The RGB image was taken by Andres Victorero\protect\footnotemark on Pexels\protect\footnotemark}
    \label{fig:two_head}
\end{figure}
\fi

%\tablefootnote{\href{https://www.pexels.com/@andres-victorero-2102935/}{https://www.pexels.com/@andres-victorero-2102935/}}
%\footnotetext[1]{Profile available at \href{https://www.pexels.com/@andres-victorero-2102935/}{https://www.pexels.com/@andres-victorero-2102935/}}
%\footnotetext[2]{Image available at \href{https://www.pexels.com/photo/blue-and-white-toy-dolphin-floating-on-water-3730754/}{https://www.pexels.com/photo/blue-and-white-toy-dolphin-floating-on-water-3730754/}}


% \paragraph{Progressive Diffusion}
% Inspired by the successes of GANs in progressive image reconstruction, we've leveraged these principles in diffusion models. As described in Subsec.~\ref{sec:diffusion_models}, diffusion models work by learning how to reverse a diffusion process that slowly adds random noise to data. Similarly to image reconstruction, the reversal diffusion process is applied to the entire image. As in progressive image reconstruction, we believe that reversing the diffusion process in a certain regions of the image could be more challenging in others. Specifically we assume reversing the process in the center of the image, where the objects are typically located could pose a bigger challenge without additional information. Therefore, we progressively mask the image during the denoising steps to first let the system focus on reversing the diffusion process in the borders of the image. The approach is depicted in Fig. 


